An elliptic local problem with exponential decay of the resonance error for numerical homogenization

Numerical multiscale methods usually rely on some coupling between a macroscopic and a microscopic model. The macroscopic model is incomplete as effective quantities, such as the homogenized material coefficients or fluxes, are missing in the model. These effective data need to be computed by running local microscale simulations followed by a local averaging of the microscopic information. Motivated by the classical homogenization theory, it is a common practice to use local elliptic cell problems for computing the missing homogenized coefficients in the macro model. Such a consideration results in a first order error $O(\varepsilon/\delta)$, where $\varepsilon$ represents the wavelength of the microscale variations and $\delta$ is the size of the microscopic simulation boxes. This error, called "resonance error", originates from the boundary conditions used in the micro-problem and typically dominates all other errors in a multiscale numerical method. Optimal decay of the resonance error remains an open problem, although several interesting approaches reducing the effect of the boundary have been proposed over the last two decades. In this paper, as an attempt to resolve this problem, we propose a computationally efficient, fully elliptic approach with exponential decay of the resonance error.

==> Figures/TwoD_Correlated_Signal_Boundary_Error.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
%
\begin{tikzpicture}

\begin{axis}[%
width=5cm,
height=3.35cm,
%at={(0.692in,0.511in)},
scale only axis,
xmode=log,
xmin=1,
xmax=12.703,
xlabel style={font=\color{white!15!black}},
xlabel={$R$},
xtick={1, 10, 20},
xticklabels={1, 10, 20},
minor xtick={1,2,3,4,5,6,7,8,9,10,20},
ymode=log,
ymin=1e-05,
ymax=1e-2,
yminorticks=false,
ylabel style={font=\color{white!15!black}},
ylabel={$\|a^{0}_{T,R,L}  - a^{0}\|_{F}$},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
%yminorgrids,
legend style={font=\scriptsize, at={(.02,.02)}, anchor = south west,legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	0.00735699108747107\\
1.17077991372278	0.00582610123914012\\
1.37072560637672	0.00534256779498827\\
1.60481800717134	0.00462156638640721\\
1.87888868797682	0.00408115486077424\\
2.19976513600421	0.00340542159367852\\
2.57544083614139	0.00278637601169742\\
3.01527439993574	0.00227559997303069\\
3.53022270180727	0.00184599070326979\\
4.13311383024411	0.00152686626861488\\
4.83896665357963	0.00118454408607683\\
5.66536496118536	0.000872116153267343\\
6.63289550046465	0.000587244977216194\\
7.76566082176622	0.000341233330903856\\
9.09187970690782	0.000166970979369202\\
10.6445901388314	8.20621149562507e-05\\
12.4624723243554	4.09696101084437e-05\\
14.5908122726813	1.64807078869809e-05\\
17.0826299337551	2.67926398676404e-06\\
};
\addlegendentry{$q=1$}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0.00768745840985337\\
1.17077991372278	0.00636565481824775\\
1.37072560637672	0.00555322305492806\\
1.60481800717134	0.00496338091943251\\
1.87888868797682	0.00439891559026702\\
2.19976513600421	0.00372322499976874\\
2.57544083614139	0.00311597399182689\\
3.01527439993574	0.00261097175135529\\
3.53022270180727	0.00219263782028739\\
4.13311383024411	0.00183829393716733\\
4.83896665357963	0.00148799881210465\\
5.66536496118536	0.0011715707435239\\
6.63289550046465	0.000882335843327407\\
7.76566082176622	0.000615022471985574\\
9.09187970690782	0.000382142137763565\\
10.6445901388314	0.000203845866611941\\
12.4624723243554	8.94041837418484e-05\\
14.5908122726813	2.95798067537707e-05\\
17.0826299337551	6.90821708137991e-06\\
};
\addlegendentry{$q=3$}

\addplot [color=mycolor3]
  table[row sep=crcr]{%
1	0.00776944756926505\\
1.17077991372278	0.00646195148685019\\
1.37072560637672	0.00565316431692581\\
1.60481800717134	0.0050546361271086\\
1.87888868797682	0.00449234488519585\\
2.19976513600421	0.00382117963438443\\
2.57544083614139	0.00322043607312358\\
3.01527439993574	0.00271375002535303\\
3.53022270180727	0.00230072525162665\\
4.13311383024411	0.00193871065985178\\
4.83896665357963	0.00158617892570599\\
5.66536496118536	0.00126763846582228\\
6.63289550046465	0.000978686817337847\\
7.76566082176622	0.000708768263426123\\
9.09187970690782	0.000467639782550843\\
10.6445901388314	0.000271256969925251\\
12.4624723243554	0.000133079714653712\\
14.5908122726813	5.17403901383759e-05\\
17.0826299337551	1.34181181137753e-05\\
};
\addlegendentry{$q=5$}

\end{axis}
\end{tikzpicture}%

==> Figures/TwoD_Ex1_q_25.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=5cm,
height=3.35cm,
%at={(0.692in,0.511in)},
scale only axis,
xmode=log,
xmin=1,
xmax=12.703,
xlabel style={font=\color{white!15!black}},
xlabel={$R$},
xtick={1, 10, 20},
xticklabels={1, 10, 20},
minor xtick={1,2,3,4,5,6,7,8,9,10,20},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\|a^{0}_{T,R,L}  - a^{0}\|_{F}$},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={font=\scriptsize, at={(.02,.02)}, anchor = south west,legend cell align=left, align=left, draw=white!15!black}
]
 \addplot [color=blue]
  table[row sep=crcr]{%
1	0.22478\\
1.0307	0.21647\\
1.0624	0.20683\\
1.095	0.19582\\
1.1287	0.18345\\
1.1633	0.16979\\
1.1991	0.15501\\
1.2359	0.13935\\
1.2739	0.12317\\
1.313	0.10694\\
1.3534	0.091204\\
1.395	0.076555\\
1.4378	0.063554\\
1.482	0.052664\\
1.5275	0.044181\\
1.5744	0.038188\\
1.6228	0.034551\\
1.6727	0.032954\\
1.7241	0.032951\\
1.777	0.034026\\
1.8316	0.035638\\
1.8879	0.037261\\
1.9459	0.038404\\
2.0057	0.038641\\
2.0673	0.037639\\
2.1308	0.035208\\
2.1963	0.031355\\
2.2637	0.026353\\
2.3333	0.020757\\
2.405	0.015351\\
2.4789	0.010957\\
2.555	0.0081678\\
2.6335	0.0071392\\
2.7144	0.007575\\
2.7978	0.0088863\\
2.8838	0.010382\\
2.9724	0.01141\\
3.0637	0.011457\\
3.1578	0.010261\\
3.2548	0.0079462\\
3.3548	0.0051143\\
3.4579	0.0027076\\
3.5641	0.0015441\\
3.6736	0.0018095\\
3.7865	0.0030203\\
3.9028	0.0043837\\
4.0227	0.0051334\\
4.1463	0.0047619\\
4.2737	0.0032759\\
4.405	0.0013917\\
4.5403	0.00021169\\
4.6798	0.00028581\\
4.8236	0.0012054\\
4.9718	0.0021389\\
5.1245	0.0023334\\
5.282	0.00152\\
5.4442	0.00030836\\
5.6115	0.00023065\\
5.7839	0.00017507\\
5.9616	0.00087171\\
6.1447	0.0010905\\
6.3335	0.00056438\\
6.5281	5.1522e-05\\
6.7287	1.427e-05\\
6.9354	0.00048804\\
7.1484	0.0006623\\
7.3681	0.00026523\\
7.5944	7.714e-05\\
7.8277	0.00012391\\
8.0682	0.00039153\\
8.3161	0.00023431\\
8.5716	4.2648e-05\\
8.8349	7.9864e-05\\
9.1064	0.0002445\\
9.3861	8.4121e-05\\
9.6745	1.7505e-05\\
9.9717	0.00015318\\
10.278	0.00015178\\
10.594	2.7336e-05\\
10.919	7.463e-05\\
11.255	0.0001119\\
11.601	2.3036e-05\\
11.957	5.6081e-05\\
12.324	5.8162e-05\\
12.703	1.4865e-05\\
};
\addlegendentry{$q=2$}

\addplot [color=blue, dashed]
  table[row sep=crcr]{%
1	0.1\\
1.0307	0.0913278369752717\\
1.0624	0.0833941936775626\\
1.095	0.0761653851364584\\
1.1287	0.0695447619472234\\
1.1633	0.0635220954023051\\
1.1991	0.0580007742606193\\
1.2359	0.0529724431170149\\
1.2739	0.0483719936470275\\
1.313	0.0441779766922005\\
1.3534	0.0403386615012337\\
1.395	0.0368364167025707\\
1.4378	0.0336437627832164\\
1.482	0.0307224176696412\\
1.5275	0.0280579762489319\\
1.5744	0.0256244620493095\\
1.6228	0.0233994151611395\\
1.6727	0.0213671121390059\\
1.7241	0.0195124877958626\\
1.777	0.0178212316973097\\
1.8316	0.0162745165174734\\
1.8879	0.0148615135092537\\
1.9459	0.0135718310855703\\
2.0057	0.0123937313061805\\
2.0673	0.0113185159215147\\
2.1308	0.0103364625542643\\
2.1963	0.00943897890036214\\
2.2637	0.00862071698221133\\
2.3333	0.00787205748569072\\
2.405	0.00718877279749683\\
2.4789	0.00656482234072841\\
2.555	0.00599552594368623\\
2.6335	0.00547520055545049\\
2.7144	0.00500009735139942\\
2.7978	0.00456614819513066\\
2.8838	0.00416969786736652\\
2.9724	0.00380783605829702\\
3.0637	0.003477453170909\\
3.1578	0.00317574877177799\\
3.2548	0.00290019418897757\\
3.3548	0.00264850072993011\\
3.4579	0.00241859255178792\\
3.5641	0.00220876930148331\\
3.6736	0.00201708593391066\\
3.7865	0.00184198511566817\\
3.9028	0.00168217475488736\\
4.0227	0.00153619753361896\\
4.1463	0.00140287131429581\\
4.2737	0.00128111436682393\\
4.405	0.00116993642277382\\
4.5403	0.00106843068086985\\
4.6798	0.000975704079347165\\
4.8236	0.000891017308518063\\
4.9718	0.000813690133567961\\
5.1245	0.000743096999322456\\
5.282	0.000678585865584599\\
5.4442	0.000619723245122883\\
5.6115	0.000565930497398675\\
5.7839	0.00051681804986566\\
5.9616	0.000471966855015394\\
6.1447	0.000431020520366045\\
6.3335	0.000393612312774983\\
6.5281	0.000359450924155968\\
6.7287	0.000328251336503144\\
6.9354	0.000299768129255618\\
7.1484	0.000273762186941818\\
7.3681	0.000249996233506596\\
7.5944	0.000228307194001159\\
7.8277	0.000208495882004869\\
8.0682	0.000190401354774264\\
8.3161	0.00017387650053384\\
8.5716	0.000158786768899617\\
8.8349	0.000145009042668166\\
9.1064	0.000132421905059059\\
9.3861	0.000120932900508098\\
9.6745	0.000110436952331721\\
9.9717	0.000100853828101783\\
10.278	9.21030813490389e-05\\
10.594	8.41046667227792e-05\\
10.919	7.68159493080519e-05\\
11.255	7.01396350753025e-05\\
11.601	6.40492014774663e-05\\
11.957	5.84969620522093e-05\\
12.324	5.34250492344593e-05\\
12.703	4.87844154756011e-05\\
};
\addlegendentry{$O(R^{-3})$}

\addplot [color=black]
  table[row sep=crcr]{%
1	0.21977\\
1.0307	0.21127\\
1.0624	0.20149\\
1.095	0.19041\\
1.1287	0.17806\\
1.1633	0.16454\\
1.1991	0.15003\\
1.2359	0.13478\\
1.2739	0.11916\\
1.313	0.1036\\
1.3534	0.088616\\
1.395	0.074716\\
1.4378	0.06238\\
1.482	0.051977\\
1.5275	0.043716\\
1.5744	0.037616\\
1.6228	0.033516\\
1.6727	0.031112\\
1.7241	0.030007\\
1.777	0.029768\\
1.8316	0.029959\\
1.8879	0.03018\\
1.9459	0.03008\\
2.0057	0.029381\\
2.0673	0.027897\\
2.1308	0.025567\\
2.1963	0.022479\\
2.2637	0.018891\\
2.3333	0.015219\\
2.405	0.011962\\
2.4789	0.0095653\\
2.555	0.0082658\\
2.6335	0.0080081\\
2.7144	0.008486\\
2.7978	0.0092649\\
2.8838	0.0099021\\
2.9724	0.010028\\
3.0637	0.0094059\\
3.1578	0.007994\\
3.2548	0.0060055\\
3.3548	0.003908\\
3.4579	0.0022784\\
3.5641	0.001506\\
3.6736	0.0015683\\
3.7865	0.0021103\\
3.9028	0.0026819\\
4.0227	0.0029071\\
4.1463	0.0025828\\
4.2737	0.0017724\\
4.405	0.00084497\\
4.5403	0.00027085\\
4.6798	0.00022042\\
4.8236	0.00048625\\
4.9718	0.0007574\\
5.1245	0.00077348\\
5.282	0.00047485\\
5.4442	8.9955e-05\\
5.6115	7.1101e-05\\
5.7839	2.8441e-05\\
5.9616	0.00018691\\
6.1447	0.00021293\\
6.3335	8.6214e-05\\
6.5281	1.6449e-06\\
6.7287	8.5986e-05\\
6.9354	0.00022086\\
7.1484	0.00022854\\
7.3681	8.5964e-05\\
7.5944	3.4635e-05\\
7.8277	2.7551e-05\\
8.0682	2.1668e-05\\
8.3161	1.4614e-05\\
8.5716	2.9558e-06\\
8.8349	4.531e-05\\
9.1064	6.2474e-05\\
9.3861	1.2351e-05\\
9.6745	3.2206e-06\\
9.9717	6.6124e-06\\
10.278	2.4699e-06\\
10.594	6.5546e-07\\
10.919	1.1919e-05\\
11.255	7.4962e-06\\
11.601	3.711e-07\\
11.957	7.7146e-06\\
12.324	2.4051e-06\\
12.703	1.8379e-06\\
};
\addlegendentry{$q=5$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
1	10\\
1.0307	8.34077380658181\\
1.0624	6.95459153913083\\
1.095	5.80116589298504\\
1.1287	4.83647391429597\\
1.1633	4.03505660429956\\
1.1991	3.36408981483131\\
1.2359	2.80607972978538\\
1.2739	2.33984976938807\\
1.313	1.95169362461661\\
1.3534	1.62720761171112\\
1.395	1.35692159548543\\
1.4378	1.13190277421333\\
1.482	0.943866947467879\\
1.5275	0.787250031185625\\
1.5744	0.656613055316505\\
1.6228	0.547532629883365\\
1.6727	0.456553481160854\\
1.7241	0.380737179983687\\
1.777	0.317596299209196\\
1.8316	0.264859887877514\\
1.8879	0.220864583785731\\
1.9459	0.184194599015254\\
2.0057	0.153604575689799\\
2.0673	0.128108802665583\\
2.1308	0.106842458135708\\
2.1963	0.0890943226814817\\
2.2637	0.0743167612873868\\
2.3333	0.0619692890580192\\
2.405	0.0516784543340304\\
2.4789	0.0430968923653268\\
2.555	0.0359463313414146\\
2.6335	0.0299778211224053\\
2.7144	0.0250009735234715\\
2.7978	0.0208497093398949\\
2.8838	0.0173863803051209\\
2.9724	0.014499615446867\\
3.0637	0.012092680555865\\
3.1578	0.0100853802614494\\
3.2548	0.00841112633377926\\
3.3548	0.00701455611644035\\
3.4579	0.00584958993156399\\
3.5641	0.00487866182717505\\
3.6736	0.00406863566478025\\
3.7865	0.00339290916634307\\
3.9028	0.00282971190598036\\
4.0227	0.00235990286229698\\
4.1463	0.00196804792447406\\
4.2737	0.00164125402088267\\
4.405	0.0013687512333328\\
4.5403	0.00114154411982401\\
4.6798	0.000951998450454699\\
4.8236	0.000793911844078774\\
4.9718	0.000662091633465846\\
5.1245	0.000552193150402038\\
5.282	0.000460478776971199\\
5.4442	0.000384056900545637\\
5.6115	0.000320277327885912\\
5.7839	0.000267100896666943\\
5.9616	0.000222752712233121\\
6.1447	0.000185778688976616\\
6.3335	0.000154930652768071\\
6.5281	0.000129204966876579\\
6.7287	0.000107748939916101\\
6.9354	8.98609313174128e-05\\
7.1484	7.49457349991666e-05\\
7.3681	6.24981167674845e-05\\
7.5944	5.21241748326828e-05\\
7.8277	4.34705328129883e-05\\
8.0682	3.62526758998752e-05\\
8.3161	3.02330374378945e-05\\
8.5716	2.52132379775803e-05\\
8.8349	2.10276224555381e-05\\
9.1064	1.75355609394705e-05\\
9.3861	1.46247664253014e-05\\
9.6745	1.21963204403188e-05\\
9.9717	1.01714946427841e-05\\
10.278	8.48297759398768e-06\\
10.594	7.07359496454977e-06\\
10.919	5.90069006809719e-06\\
11.255	4.9195684084966e-06\\
11.601	4.10230020990108e-06\\
11.957	3.42189456933762e-06\\
12.324	2.8542358857044e-06\\
12.703	2.37991919329607e-06\\
};
\addlegendentry{$O(R^{-6})$}

\end{axis}
\end{tikzpicture}%

==> Figures/TwoD_Layered_q_25.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=5cm,
height=3.35cm,
%at={(0.692in,0.511in)},
scale only axis,
xmode=log,
xmin=1,
xmax=12.703,
xlabel style={font=\color{white!15!black}},
xlabel={$R$},
xtick={1, 10, 20},
xticklabels={1, 10, 20},
minor xtick={1,2,3,4,5,6,7,8,9,10,20},
ymode=log,
ymin=1e-07,
ymax=1,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={$\|a^{0}_{T,R,L}  - a^{0}\|_{F}$},
axis background/.style={fill=white},
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
legend style={font=\scriptsize, at={(.02,.02)}, anchor = south west,legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue]
  table[row sep=crcr]{%
1	0.064855825814373\\
1.03072240652209	0.06540010043088\\
1.06238867930668	0.0670261575135309\\
1.09502781619681	0.0665117396359582\\
1.128669705919	0.0667824675655903\\
1.1633451554534	0.0668094404336722\\
1.19908591824474	0.0674774130047439\\
1.23592472327997	0.0670851173647957\\
1.27389530505927	0.0664862179864802\\
1.31303243448788	0.0649398688384608\\
1.35337195071691	0.0635586318634312\\
1.39495079396242	0.0620275113051366\\
1.43780703933284	0.0597457259737172\\
1.48197993169554	0.0578259826305351\\
1.52750992161467	0.0550439306284099\\
1.57443870239304	0.053380578525071\\
1.62280924825206	0.0507855850995523\\
1.67266585368467	0.0481637603231869\\
1.72405417401718	0.0446169684525993\\
1.77702126721744	0.0405102389539126\\
1.83161563698728	0.0376994860088103\\
1.88788727717902	0.0333155724836048\\
1.94588771757639	0.0303949320815282\\
2.00567007108211	0.0263481900243228\\
2.06728908235507	0.0226248496197859\\
2.13080117794186	0.0190243075166442\\
2.19626451794833	0.0157751852940636\\
2.26373904929878	0.0116500769772599\\
2.33328656063125	0.00874380545716436\\
2.40497073887949	0.00643743098896299\\
2.47885722759307	0.00421471111838784\\
2.5550136870494	0.00202413852307282\\
2.63350985621243	8.11689283001793e-05\\
2.71441761659491	0.00157501877210059\\
2.79781105808265	0.00262893310981588\\
2.88376654678106	0.00327908134220301\\
2.97236279494606	0.00428738545335966\\
3.06368093306352	0.0046997527543865\\
3.15780458414306	0.00498331735577023\\
3.25481994029442	0.00507188590839519\\
3.35481584165634	0.00496568992169089\\
3.45788385775044	0.00488679782963647\\
3.56411837133441	0.00441013415498348\\
3.67361666483139	0.00397395269753736\\
3.78647900941465	0.0034993652252272\\
3.90280875682923	0.00287784953450909\\
4.0227124340345	0.00223897376997878\\
4.14629984075437	0.00173149119737565\\
4.27368415002449	0.00102241319649371\\
4.40498201182854	0.0002782212635416\\
4.54031365991841	0.000420568431003576\\
4.67980302191621	0.00089875337238815\\
4.82357783279881	0.0014843920447819\\
4.97176975186899	0.0018045362394723\\
5.12451448332012	0.00178889511980757\\
5.281951900505	0.00163367305989498\\
5.44422617402243	0.0013188466495368\\
5.61148590373893	0.000879306080428965\\
5.78388425486656	0.000416217942136365\\
5.96157909822127	0.000158831377424618\\
6.1447331547904	0.000546596028231316\\
6.33351414474162	0.0008670376547949\\
6.52809494100976	0.000939814373426329\\
6.72865372760224	0.000839037599542569\\
6.93537416276799	0.000587545195175065\\
7.14844554717933	0.000284050395321755\\
7.36806299728077	2.29507760564629e-05\\
7.59442762396358	0.000246943217029283\\
7.82774671672956	0.000389556215356468\\
8.06823393351286	0.000406177526778628\\
8.31610949633354	0.000312877946439805\\
8.57160039296208	0.000222802995255844\\
8.83494058477954	4.21444277985406e-05\\
9.10637122102363	0.000117348936918782\\
9.38614085961695	0.000200557095516418\\
9.67450569477967	0.000228459497554068\\
9.97172979163494	0.000210148352218775\\
10.2780853280219	8.78998470765224e-05\\
10.5938528437381	1.43770012309141e-05\\
10.9193214974386	0.000148900014470876\\
11.2547893314283	0.000166931192157993\\
11.6005635445889	0.000110515128251887\\
11.9569607736911	1.14493834534879e-05\\
12.324307383349	0.000100884044801797\\
12.7029397648834	0.000121065463693892\\
};
\addlegendentry{$q=2$}

\addplot [color=blue, dashed]
  table[row sep=crcr]{%
1	0.0999999999999999\\
1.03072240652209	0.0913218810708524\\
1.06238867930668	0.0833968596231893\\
1.09502781619681	0.0761595809619147\\
1.128669705919	0.0695503619500994\\
1.1633451554534	0.0635146988244172\\
1.19908591824474	0.0580028177229444\\
1.23592472327997	0.0529692642186907\\
1.27389530505927	0.0483725284738983\\
1.31303243448788	0.0441747029238977\\
1.35337195071691	0.0403411696675643\\
1.39495079396242	0.0368403149864038\\
1.43780703933284	0.0336432686380112\\
1.48197993169554	0.030723665773952\\
1.52750992161467	0.0280574295186947\\
1.57443870239304	0.0256225724166006\\
1.62280924825206	0.0233990151095811\\
1.67266585368467	0.0213684207501224\\
1.72405417401718	0.0195140437841462\\
1.77702126721744	0.017820591856672\\
1.83161563698728	0.0162740997014721\\
1.88788727717902	0.0148618139747303\\
1.94588771757639	0.0135720880829745\\
2.00567007108211	0.0123942861379653\\
2.06728908235507	0.0113186952464939\\
2.13080117794186	0.0103364454117754\\
2.19626451794833	0.00943943638589509\\
2.26373904929878	0.00862027087008589\\
2.33328656063125	0.00787219351196518\\
2.40497073887949	0.00718903519666421\\
2.47885722759307	0.00656516217243942\\
2.5550136870494	0.00599542959122372\\
2.63350985621243	0.00547513908098403\\
2.71441761659491	0.005\\
2.79781105808265	0.00456609405354262\\
2.88376654678106	0.00416984298115946\\
2.97236279494606	0.00380797904809573\\
3.06368093306352	0.00347751809750497\\
3.15780458414306	0.00317573494122086\\
3.25481994029442	0.00290014088614722\\
3.35481584165634	0.00264846321093453\\
3.45788385775044	0.00241862642369492\\
3.56411837133441	0.00220873514619488\\
3.67361666483139	0.00201705848337821\\
3.78647900941465	0.00184201574932019\\
3.90280875682923	0.00168216343190056\\
4.0227124340345	0.0015361832886976\\
4.14629984075437	0.00140287147593473\\
4.27368415002449	0.00128112862083003\\
4.40498201182854	0.00116995075547905\\
4.54031365991841	0.00106842103750612\\
4.67980302191621	0.000975702189207308\\
4.82357783279881	0.000891029592833602\\
4.97176975186899	0.000813704985073604\\
5.12451448332012	0.000743090698736514\\
5.281951900505	0.000678604404148726\\
5.44422617402243	0.000619714306898267\\
5.61148590373893	0.000565934762324693\\
5.78388425486656	0.000516822270588769\\
5.96157909822127	0.000471971819294755\\
6.1447331547904	0.000431013543504295\\
6.33351414474162	0.000393609675598259\\
6.52809494100976	0.00035945175983321\\
6.72865372760224	0.000328258108621971\\
6.93537416276799	0.000299771479561186\\
7.14844554717933	0.000273756954049201\\
7.36806299728077	0.00025\\
7.59442762396358	0.000228304702677131\\
7.82774671672956	0.000208492149057973\\
8.06823393351286	0.000190398952404787\\
8.31610949633354	0.000173875904875248\\
8.57160039296208	0.000158786747061043\\
8.83494058477954	0.000145007044307361\\
9.10637122102363	0.000132423160546727\\
9.38614085961695	0.000120931321184746\\
9.67450569477967	0.000110436757309744\\
9.97172979163494	0.000100852924168911\\
10.2780853280219	9.21007874660097e-05\\
10.5938528437381	8.41081715950279e-05\\
10.9193214974386	7.680916443488e-05\\
11.2547893314283	7.01435737967366e-05\\
11.6005635445889	6.40564310415015e-05\\
11.9569607736911	5.84975377739526e-05\\
12.324307383349	5.3421051875306e-05\\
12.7029397648834	4.87851094603654e-05\\
};
\addlegendentry{$O(R^{-3})$}

\addplot [color=black]
  table[row sep=crcr]{%
1	0.0820949982981397\\
1.03072240652209	0.0832389752215932\\
1.06238867930668	0.0850900615798841\\
1.09502781619681	0.085465283168598\\
1.128669705919	0.087012596056815\\
1.1633451554534	0.08797351552122\\
1.19908591824474	0.0891974634191951\\
1.23592472327997	0.0898620239905188\\
1.27389530505927	0.0903347900461185\\
1.31303243448788	0.0900165373147566\\
1.35337195071691	0.0897255626088907\\
1.39495079396242	0.0890423293704338\\
1.43780703933284	0.0885842370232774\\
1.48197993169554	0.0875420139623781\\
1.52750992161467	0.0865358398446801\\
1.57443870239304	0.0864785700097965\\
1.62280924825206	0.0852840735508729\\
1.67266585368467	0.083972156415605\\
1.72405417401718	0.0818429596136406\\
1.77702126721744	0.0787249176331056\\
1.83161563698728	0.0769182920500113\\
1.88788727717902	0.0740993982665442\\
1.94588771757639	0.072729963679519\\
2.00567007108211	0.0692693568403042\\
2.06728908235507	0.0665673792598733\\
2.13080117794186	0.0638239196470096\\
2.19626451794833	0.061741875859222\\
2.26373904929878	0.0577282658115155\\
2.33328656063125	0.0555497502604449\\
2.40497073887949	0.0523999894694768\\
2.47885722759307	0.0496427233170926\\
2.5550136870494	0.0467755028312054\\
2.63350985621243	0.0443992377080855\\
2.71441761659491	0.0408927985346574\\
2.79781105808265	0.038652333642869\\
2.88376654678106	0.0360463698253148\\
2.97236279494606	0.0328612573244975\\
3.06368093306352	0.0295853387849494\\
3.15780458414306	0.0273066799905083\\
3.25481994029442	0.0240550173194199\\
3.35481584165634	0.021335918809311\\
3.45788385775044	0.0190342979601414\\
3.56411837133441	0.0160515389149448\\
3.67361666483139	0.0138704748505374\\
3.78647900941465	0.0115574292942178\\
3.90280875682923	0.00927869735346026\\
4.0227124340345	0.00748848960621296\\
4.14629984075437	0.00563224090360315\\
4.27368415002449	0.0042352755010846\\
4.40498201182854	0.00296224025844316\\
4.54031365991841	0.00194445599014603\\
4.67980302191621	0.00112860038266471\\
4.82357783279881	0.000562335321536878\\
4.97176975186899	0.0001317444982466\\
5.12451448332012	0.000203266052201834\\
5.281951900505	0.000523566647104401\\
5.44422617402243	0.00061779652657501\\
5.61148590373893	0.000510916303027853\\
5.78388425486656	0.000440045171677117\\
5.96157909822127	0.000420669715394228\\
6.1447331547904	0.000436861622755635\\
6.33351414474162	0.000192145631019491\\
6.52809494100976	0.000133526048402555\\
6.72865372760224	4.41946810569305e-05\\
6.93537416276799	3.43005592413625e-05\\
7.14844554717933	8.0174938259292e-05\\
7.36806299728077	9.71145504429782e-05\\
7.59442762396358	0.00015290485008429\\
7.82774671672956	6.47254760292593e-05\\
8.06823393351286	3.12168462667239e-05\\
8.31610949633354	2.55245620478517e-06\\
8.57160039296208	8.57860328529192e-06\\
8.83494058477954	2.11170243865633e-05\\
9.10637122102363	2.3185684149718e-05\\
9.38614085961695	1.47618926590876e-05\\
9.67450569477967	7.70527193755255e-06\\
9.97172979163494	8.62777737559162e-06\\
10.2780853280219	4.79410680925829e-06\\
10.5938528437381	2.80714412952965e-05\\
10.9193214974386	2.93962881676157e-05\\
11.2547893314283	4.23028765417222e-06\\
11.6005635445889	2.00471306993633e-06\\
11.9569607736911	2.96428940433358e-05\\
12.324307383349	1.3010789893797e-06\\
12.7029397648834	3.10213801313353e-07\\
};
\addlegendentry{$q=5$}

\addplot [color=black, dashed]
  table[row sep=crcr]{%
1	9.99999999999999\\
1.03072240652209	8.33968596231892\\
1.06238867930668	6.95503619500993\\
1.09502781619681	5.80028177229444\\
1.128669705919	4.83725284738983\\
1.1633451554534	4.03411696675642\\
1.19908591824474	3.36432686380112\\
1.23592472327997	2.80574295186946\\
1.27389530505927	2.3399015109581\\
1.31303243448788	1.95140437841462\\
1.35337195071691	1.62740997014721\\
1.39495079396242	1.35720880829745\\
1.43780703933284	1.13186952464939\\
1.48197993169554	0.943943638589509\\
1.52750992161467	0.787219351196518\\
1.57443870239304	0.656516217243941\\
1.62280924825206	0.547513908098402\\
1.67266585368467	0.456609405354262\\
1.72405417401718	0.380797904809573\\
1.77702126721744	0.317573494122086\\
1.83161563698728	0.264846321093453\\
1.88788727717902	0.220873514619488\\
1.94588771757639	0.184201574932019\\
2.00567007108211	0.15361832886976\\
2.06728908235507	0.128112862083003\\
2.13080117794186	0.106842103750612\\
2.19626451794833	0.0891029592833602\\
2.26373904929878	0.0743090698736514\\
2.33328656063125	0.0619714306898267\\
2.40497073887949	0.0516822270588768\\
2.47885722759307	0.0431013543504294\\
2.5550136870494	0.035945175983321\\
2.63350985621243	0.0299771479561186\\
2.71441761659491	0.025\\
2.79781105808265	0.0208492149057973\\
2.88376654678106	0.0173875904875248\\
2.97236279494606	0.0145007044307361\\
3.06368093306352	0.0120931321184746\\
3.15780458414306	0.0100852924168911\\
3.25481994029442	0.00841081715950279\\
3.35481584165634	0.00701435737967365\\
3.45788385775044	0.00584975377739526\\
3.56411837133441	0.00487851094603654\\
3.67361666483139	0.00406852492536801\\
3.78647900941465	0.00339302202074363\\
3.90280875682923	0.00282967381162346\\
4.0227124340345	0.00235985909647377\\
4.14629984075437	0.00196804837799129\\
4.27368415002449	0.00164129054310985\\
4.40498201182854	0.001368784770246\\
4.54031365991841	0.00114152351338566\\
4.67980302191621	0.000951994762023933\\
4.82357783279881	0.000793933735305215\\
4.97176975186899	0.000662115802733633\\
5.12451448332012	0.000552183786548721\\
5.281951900505	0.000460503937330048\\
5.44422617402243	0.0003840458221744\\
5.61148590373893	0.000320282155207507\\
5.78388425486656	0.00026710525937653\\
5.96157909822127	0.0002227573982084\\
6.1447331547904	0.000185772674684128\\
6.33351414474162	0.000154928576724567\\
6.52809494100976	0.000129205567647192\\
6.72865372760224	0.000107753385876074\\
6.93537416276799	8.98629399583026e-05\\
7.14844554717933	7.49428698902965e-05\\
7.36806299728077	6.24999999999999e-05\\
7.59442762396358	5.21230372644932e-05\\
7.82774671672956	4.34689762188121e-05\\
8.06823393351286	3.62517610768402e-05\\
8.31610949633354	3.02328302961864e-05\\
8.57160039296208	2.52132310422276e-05\\
8.83494058477954	2.1027042898757e-05\\
9.10637122102363	1.75358934491841e-05\\
9.38614085961695	1.46243844434881e-05\\
9.67450569477967	1.21962773650913e-05\\
9.97172979163494	1.017131231342e-05\\
10.2780853280219	8.48255505185908e-06\\
10.5938528437381	7.07418452905866e-06\\
10.9193214974386	5.89964774118443e-06\\
11.2547893314283	4.92012094497823e-06\\
11.6005635445889	4.10322635777464e-06\\
11.9569607736911	3.42196192561501e-06\\
12.324307383349	2.85380878346414e-06\\
12.7029397648834	2.37998690505983e-06\\
};
\addlegendentry{$O(R^{-6})$}

\end{axis}
\end{tikzpicture}%

==> tex/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Local problem with exponential decay of the resonance error}{A. Abdulle, D. Arjmand, and E. Paganoni}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An elliptic local problem with exponential decay of the resonance error for numerical homogenization %\del{problems}
	\thanks{Submitted to the editors DATE.}
	}

% Authors: full names plus addresses.
\author{
	Assyr Abdulle\thanks{ ANMC, Institute of Mathematics, {\'E}cole Polytechnique F{\'e}d{\'e}rale de Lausanne, Station 8, CH 1015 Lausanne, Switzerland
		(\email{assyr.abdulle@epfl.ch}, \email{edoardo.paganoni@epfl.ch}).}
	\and
	Doghonay Arjmand\footnotemark[2] \thanks{Division of Applied Mathematics, School of Education, Culture and Communication, M{\"a}lardalen University, Box 883, 721 23, V{\"a}ster{\aa}s, Sweden
		(\email{doghonay.arjmand@mdh.se}).} 
	\and
	Edoardo Paganoni\footnotemark[2]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

